Efficient Motion Prediction: A Lightweight & Accurate Trajectory Prediction Model With Fast Training and Inference Speed

For efficient and safe autonomous driving, it is essential that autonomous vehicles can predict the motion of other traffic agents. While highly accurate, current motion prediction models often impose significant challenges in terms of training resource requirements and deployment on embedded hardware. We propose a new efficient motion prediction model, which achieves highly competitive benchmark results while training only a few hours on a single GPU. Due to our lightweight architectural choices and the focus on reducing the required training resources, our model can easily be applied to custom datasets. Furthermore, its low inference latency makes it particularly suitable for deployment in autonomous applications with limited computing resources.

==> chapters/07_app.tex <==
Appendixes should appear before the acknowledgment.

==> chapters/08_ack.tex <==
blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub blub
